Study of ttH (H -> mu mu) in the three lepton channel at sqrt(s) = 14 TeV; A Snowmass white paper

The H -> mu mu signature provides excellent mass resolution for Higgs bosons, and is therefore an important Higgs boson decay channel despite the small dimuon branching ratio. We present an optimization of selection criteria in a search for trilepton ttH (H -> mu mu) events, in which the top quark pair decays semi-leptonically, at a simulated High Luminosity LHC (HL-LHC) running at 14 TeV. The study is performed with 3000 fb^(-1) of simulated data with an average pileup of < mu > = 140. In this ultimate HL-LHC data set, we find that ttH (H -> mu mu) will be a very difficult signature to observe due to the very small expected signal.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = ttH_mumu

default: testpdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

ps:
	latex  ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvips  ${BASENAME} -o ${BASENAME}.ps

pdf:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


